SCW Codes for Optimal CSI-Free Detection in Diffusive Molecular Communications

Instantaneous or statistical channel state information (CSI) is needed for most detection schemes developed in the molecular communication (MC) literature. Since the MC channel changes, e.g., due to variations in the velocity of flow, the temperature, or the distance between transmitter and receiver, CSI acquisition has to be conducted repeatedly to keep track of CSI variations. Frequent CSI acquisition may entail a large overhead whereas infrequent CSI acquisition may result in a low CSI estimation quality. To cope with these issues, we design codes which facilitate maximum likelihood sequence detection at the receiver without instantaneous or statistical CSI. In particular, assuming concentration shift keying modulation, we show that a class of codes, referred to as strongly constant-weight (SCW) codes, enables optimal CSI-free sequence detection at the cost of decreasing the data rate. For the proposed SCW codes, we analyze the code rate and the error rate. Simulation results verify our analytical derivations and reveal that the proposed CSI-free detector for SCW codes outperforms the baseline coherent and non-coherent detectors for uncoded transmission.

==> Fig/BER_K/BER_K.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA Sub-Optimal CSI-Free Detector (Uncoded Transmission) [5]}%
\psfrag{013}[cl][cl]{\matlabtextA Optimal Coherent Detector (Uncoded Transmission) [6]}%
\psfrag{014}[cl][cl]{\matlabtextA Optimal Non-Coherent Detector (Uncoded Transmission) [5]}%
\psfrag{015}[cl][cl]{\matlabtextA Proposed Optimal CSI-Free Detector (Coded Transmission)}%
\psfrag{016}[cl][cl]{\matlabtextA $R=[\frac{1}{2},\frac{1}{3},\frac{1}{4}]$}%
\psfrag{017}[bc][bc]{\matlabtextA BER}%
\psfrag{018}[tc][tc]{\matlabtextA Codeword/Block Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2$}%
\psfrag{001}[ct][ct]{\matlabtextA $4$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $8$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $12$}%
\psfrag{006}[ct][ct]{\matlabtextA $14$}%
\psfrag{007}[ct][ct]{\matlabtextA $16$}%
\psfrag{008}[ct][ct]{\matlabtextA $18$}%
\psfrag{009}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{-1}$}%
%
%% </ytick>

==> Fig/CER_SCW/CER_SCW.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[5,0,1]^{\mathsf{T}}$}%
\psfrag{011}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[3,0,3]^{\mathsf{T}}$}%
\psfrag{012}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[1,2,3]^{\mathsf{T}}$}%
\psfrag{013}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[3,2,1]^{\mathsf{T}}$}%
\psfrag{014}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[2,2,2]^{\mathsf{T}}$}%
\psfrag{015}[cl][cl]{\matlabtextA Upper Bounds}%
\psfrag{016}[cl][cl]{\matlabtextA Analytical}%
\psfrag{017}[cl][cl]{\matlabtextA Results}%
\psfrag{018}[cl][cl]{\matlabtextA Simulation}%
\psfrag{019}[bc][bc]{\matlabtextA CER}%
\psfrag{020}[tc][tc]{\matlabtextA SNR (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
\psfrag{004}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/CER_SNR/CER_SNR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA Lower Bound (Proposition 3)}%
\psfrag{015}[cl][cl]{\matlabtextA Upper Bound (Proposition 3)}%
\psfrag{016}[cl][cl]{\matlabtextA Upper Bound (Corollary 2)}%
\psfrag{017}[cl][cl]{\matlabtextA Upper Bound (Proposition 2)}%
\psfrag{018}[cl][cl]{\matlabtextA Simulation}%
\psfrag{019}[cl][cl]{\matlabtextA Full Binary CW Code}%
\psfrag{020}[cl][cl]{\matlabtextA with Rate $R=0.5$}%
\psfrag{021}[cl][cl]{\matlabtextA Binary CW Code}%
\psfrag{022}[bc][bc]{\matlabtextA CER}%
\psfrag{023}[tc][tc]{\matlabtextA SNR (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $1$}%
\psfrag{002}[ct][ct]{\matlabtextA $2$}%
\psfrag{003}[ct][ct]{\matlabtextA $3$}%
\psfrag{004}[ct][ct]{\matlabtextA $4$}%
\psfrag{005}[ct][ct]{\matlabtextA $5$}%
\psfrag{006}[ct][ct]{\matlabtextA $6$}%
\psfrag{007}[ct][ct]{\matlabtextA $7$}%
\psfrag{008}[ct][ct]{\matlabtextA $8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{012}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{013}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>
